SpotNet - Learned iterations for cell detection in image-based immunoassays

Accurate cell detection and counting in the image-based ELISpot and FluoroSpot immunoassays is a challenging task. Recently proposed methodology matches human accuracy by leveraging knowledge of the underlying physical process of these assays and using proximal optimization methods to solve an inverse problem. Nonetheless, thousands of computationally expensive iterations are often needed to reach a near-optimal solution. In this paper, we exploit the structure of the iterations to design a parameterized computation graph, SpotNet, that learns the patterns embedded within several training images and their respective cell information. Further, we compare SpotNet to a convolutional neural network layout customized for cell detection. We show empirical evidence that, while both designs obtain a detection performance on synthetic data far beyond that of a human expert, SpotNet is easier to train and obtains better estimates of particle secretion for each cell.

==> figs/MSE_results.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.203921568627451,0.541176470588235,0.741176470588235}
\definecolor{color1}{rgb}{0.596078431372549,0.556862745098039,0.835294117647059}

\begin{axis}[
axis background/.style={fill=white!89.80392156862746!black},
axis line style={white},
tick align=outside,
tick pos=left,
title={MSE},
x grid style={white},
xmajorgrids,
xmin=0.5, xmax=2.5,
xminorgrids,
xtick={1,2},
xticklabels={SpotNet $5\times 5$,ConvNet $5\times 5$},
y grid style={white},
ymajorgrids,
ymin=200, ymax=2000,
yminorgrids
]
\addplot [black, forget plot]
table [row sep=\\]{%
0.925	465.537841907406 \\
1.075	465.537841907406 \\
1.075	622.255054139163 \\
0.925	622.255054139163 \\
0.925	465.537841907406 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1	465.537841907406 \\
1	386.380992235547 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1	622.255054139163 \\
1	662.338396277441 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
0.9625	386.380992235547 \\
1.0375	386.380992235547 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
0.9625	662.338396277441 \\
1.0375	662.338396277441 \\
};
\addplot [black, mark=x, mark size=3, mark options={solid,fill opacity=0}, only marks, forget plot]
table [row sep=\\]{%
1	371.309487590004 \\
1	344.457311039467 \\
1	327.793108147659 \\
1	341.19264482169 \\
1	383.011632691107 \\
1	329.372469015289 \\
1	355.261977699138 \\
1	301.980405421624 \\
1	355.892736662058 \\
1	309.137028507265 \\
1	379.439406766405 \\
1	332.673260078804 \\
1	381.232917791638 \\
1	361.763225647003 \\
1	308.189498975352 \\
1	683.454480817845 \\
1	714.622127439401 \\
1	677.419387908248 \\
1	692.528502920622 \\
1	704.201920589072 \\
1	813.005530759816 \\
1	662.695667833273 \\
1	704.422107318418 \\
1	669.392690389817 \\
1	781.26531735278 \\
1	738.398542913141 \\
1	694.799352773159 \\
1	752.395691566497 \\
1	676.997852732728 \\
1	702.913873300358 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1.925	1025.439631143 \\
2.075	1025.439631143 \\
2.075	1334.44458031024 \\
1.925	1334.44458031024 \\
1.925	1025.439631143 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
2	1025.439631143 \\
2	915.868842679265 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
2	1334.44458031024 \\
2	1463.01855796749 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1.9625	915.868842679265 \\
2.0375	915.868842679265 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1.9625	1463.01855796749 \\
2.0375	1463.01855796749 \\
};
\addplot [black, mark=x, mark size=3, mark options={solid,fill opacity=0}, only marks, forget plot]
table [row sep=\\]{%
2	853.919341625797 \\
2	843.183706965714 \\
2	707.963215350935 \\
2	746.21227340565 \\
2	837.356577657166 \\
2	761.179238857815 \\
2	656.879010956964 \\
2	832.227028534921 \\
2	882.843486074756 \\
2	761.209548885781 \\
2	890.56629302798 \\
2	643.102642785651 \\
2	870.026690307455 \\
2	911.28209140513 \\
2	907.837023636585 \\
2	2254.6270777611 \\
2	1483.22405437115 \\
2	1480.22208527229 \\
2	1636.35661390887 \\
2	1780.41142889174 \\
2	1652.8534597348 \\
2	1482.49452383345 \\
2	1585.23417966965 \\
2	1516.43924310494 \\
2	1484.75195905914 \\
2	1717.78561905625 \\
2	1643.56391539098 \\
2	1533.74206019701 \\
2	1497.3110693821 \\
2	1577.81725203656 \\
};
\addplot [color0, forget plot]
table [row sep=\\]{%
0.925	539.969755104348 \\
1.075	539.969755104348 \\
};
\addplot [color1, dashed, forget plot]
table [row sep=\\]{%
0.925	538.19854104976 \\
1.075	538.19854104976 \\
};
\addplot [color0, forget plot]
table [row sep=\\]{%
1.925	1205.39122641264 \\
2.075	1205.39122641264 \\
};
\addplot [color1, dashed, forget plot]
table [row sep=\\]{%
1.925	1189.68665208323 \\
2.075	1189.68665208323 \\
};
\end{axis}

\end{tikzpicture}

==> figs/detection_comparison.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.203921568627451,0.541176470588235,0.741176470588235}
\definecolor{color1}{rgb}{0.596078431372549,0.556862745098039,0.835294117647059}

\begin{axis}[
axis background/.style={fill=white!89.80392156862746!black},
axis line style={white},
tick align=outside,
tick pos=left,
title={F1-Score ratio},
x grid style={white},
xmajorgrids,
xmin=0.5, xmax=1.5,
xminorgrids,
xtick={1},
xticklabels={SpotNet over ConvNet},
y grid style={white},
ymajorgrids,
ymin=0.99584602801116, ymax=1.03857884203972,
yminorgrids
]
\addplot [black, forget plot]
table [row sep=\\]{%
0.925	1.00290582783758 \\
1.075	1.00290582783758 \\
1.075	1.01081599659396 \\
0.925	1.01081599659396 \\
0.925	1.00290582783758 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1	1.00290582783758 \\
1	1.00070426590003 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1	1.01081599659396 \\
1	1.01976325742483 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
0.9625	1.00070426590003 \\
1.0375	1.00070426590003 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
0.9625	1.01976325742483 \\
1.0375	1.01976325742483 \\
};
\addplot [black, mark=x, mark size=3, mark options={solid,fill opacity=0}, only marks, forget plot]
table [row sep=\\]{%
1	0.99793439630804 \\
1	0.998698726982188 \\
1	0.997924587190015 \\
1	0.99928370015774 \\
1	0.99793316725592 \\
1	0.998129682679028 \\
1	0.998002802359944 \\
1	0.999208708147135 \\
1	0.999661640149508 \\
1	0.998834930011402 \\
1	0.997788428648822 \\
1	0.999836501010085 \\
1	1.00009950640123 \\
1	0.998905517821247 \\
1	1.00063548938736 \\
1	1.02328362431237 \\
1	1.02513777843759 \\
1	1.0233553232397 \\
1	1.02732618643374 \\
1	1.03017241568746 \\
1	1.03613153031941 \\
1	1.03663644140206 \\
1	1.02745178597972 \\
1	1.02363971202206 \\
1	1.02841625620406 \\
1	1.02214105763392 \\
1	1.02531645726535 \\
1	1.02329625510987 \\
1	1.02458195228909 \\
1	1.02141498141476 \\
};
\addplot [color0, forget plot]
table [row sep=\\]{%
0.925	1.0065047807778 \\
1.075	1.0065047807778 \\
};
\addplot [color1, dashed, forget plot]
table [row sep=\\]{%
0.925	1.00835593365226 \\
1.075	1.00835593365226 \\
};
\end{axis}

\end{tikzpicture}

==> figs/recovery_vs_sigma.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\begin{axis}[
axis background/.style={fill=white!89.80392156862746!black},
axis line style={white},
legend cell align={left},
style = {font=\small},
legend entries={{SpotNet},{ConvNet},{True}},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={A cell's generation profile},
x grid style={white},
xtick = {9.71547043, 20.40328864, 31.15773151, 41.87789043, 52.62426725},
xticklabels = {5, 10, 15, 20, 25},
xmajorgrids,
xlabel = {$k$},
ylabel = {$(x_k[m,n])$ for a fixed $(m,n)$},
xmin=-3.114265229, xmax=65.399569809,
y grid style={white},
ymajorgrids,
ymin=-87.1844482421875, ymax=1830.87341308594,
scaled y ticks = base 10:-3,
y tick label style={
        /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        /tikz/.cd
    },
]
\addlegendimage{no markers, blue}
\addlegendimage{no markers, red}
\addlegendimage{no markers, black}
\addplot [const plot, semithick, blue, opacity=0.7]
table [row sep=\\]{%
0	772.693420410156 \\
2.03803742	789.980285644531 \\
4.07607485	896.472534179688 \\
6.44484021	854.443359375 \\
8.64666049	868.988647460938 \\
10.78428037	885.372131347656 \\
12.88968043	916.778686523438 \\
14.97645529	977.948913574219 \\
17.17280857	1027.53063964844 \\
19.33452064	1048.88256835938 \\
21.47205663	1086.0693359375 \\
23.59198881	1162.32580566406 \\
25.77936086	1192.82727050781 \\
27.94416127	1254.69848632812 \\
30.09126194	1287.14916992188 \\
32.22420107	1313.81811523438 \\
34.34561714	1344.45825195312 \\
36.5144422	1279.09777832031 \\
38.66904129	1176.12268066406 \\
40.8116676	1033.8798828125 \\
42.94411325	923.001342773438 \\
45.1138815	756.060852050781 \\
47.27192547	573.575927734375 \\
49.41978111	421.113494873047 \\
51.55872171	230.937393188477 \\
53.68981279	90.0351028442383 \\
55.8511504	57.2913055419922 \\
58.00356193	16.1712265014648 \\
60.14800566	3.83277702331543 \\
62.28530458	7.48542594909668 \\
};
\addplot [const plot, semithick, red, opacity=0.7]
table [row sep=\\]{%
0	1257.07092285156 \\
2.03803742	1235.04919433594 \\
4.07607485	1366.32202148438 \\
6.44484021	1376.04309082031 \\
8.64666049	2.33349609375 \\
10.78428037	2.39878082275391 \\
12.88968043	1448.93151855469 \\
14.97645529	1460.42785644531 \\
17.17280857	2.76766586303711 \\
19.33452064	2.88798522949219 \\
21.47205663	1517.54833984375 \\
23.59198881	1595.29333496094 \\
25.77936086	3.36822891235352 \\
27.94416127	3.53868865966797 \\
30.09126194	3.70393371582031 \\
32.22420107	3.86727142333984 \\
34.34561714	1383.73486328125 \\
36.5144422	1046.95556640625 \\
38.66904129	586.697937011719 \\
40.8116676	156.109176635742 \\
42.94411325	2.90254592895508 \\
45.1138815	2.453369140625 \\
47.27192547	0 \\
49.41978111	0 \\
51.55872171	1.08543395996094 \\
53.68981279	0.745010375976562 \\
55.8511504	0 \\
58.00356193	0 \\
60.14800566	0 \\
62.28530458	0 \\
};
\addplot [const plot,semithick, black]
table [row sep=\\]{%
0	1313.45532226562 \\
2.03803742	1308.22619628906 \\
4.07607485	1414.6064453125 \\
6.44484021	1375.67016601562 \\
8.64666049	1372.53918457031 \\
10.78428037	1383.72998046875 \\
12.88968043	1403.2216796875 \\
14.97645529	1470.701171875 \\
17.17280857	1494.37109375 \\
19.33452064	1524.06750488281 \\
21.47205663	1558.20373535156 \\
23.59198881	1626.73986816406 \\
25.77936086	1664.24450683594 \\
27.94416127	1703.65368652344 \\
30.09126194	1743.68896484375 \\
32.22420107	1339.83703613281 \\
34.34561714	330.409545898438 \\
36.5144422	0 \\
38.66904129	0 \\
40.8116676	0 \\
42.94411325	0 \\
45.1138815	0 \\
47.27192547	0 \\
49.41978111	0 \\
51.55872171	0 \\
53.68981279	0 \\
55.8511504	0 \\
58.00356193	0 \\
60.14800566	0 \\
62.28530458	0 \\
};
\end{axis}

\end{tikzpicture}
